SLAM3R: Real-Time Dense Scene Reconstruction from Monocular RGB Videos

In this paper, we introduce SLAM3R, a novel and effective system for real-time, high-quality, dense 3D reconstruction using RGB videos. SLAM3R provides an end-to-end solution by seamlessly integrating local 3D reconstruction and global coordinate registration through feed-forward neural networks. Given an input video, the system first converts it into overlapping clips using a sliding window mechanism. Unlike traditional pose optimization-based methods, SLAM3R directly regresses 3D pointmaps from RGB images in each window and progressively aligns and deforms these local pointmaps to create a globally consistent scene reconstruction - all without explicitly solving any camera parameters. Experiments across datasets consistently show that SLAM3R achieves state-of-the-art reconstruction accuracy and completeness while maintaining real-time performance at 20+ FPS. Code available at: https://github.com/PKU-VCL-3DV/SLAM3R.

==> tab/fps.tex <==
\begin{table}[tbh!]
\centering
\resizebox{0.48\textwidth}{!}{
\tiny 

\begin{tabular}{l|cccc}
\toprule

& DROID-SLAM~\cite{teed2021droid} 
& GO-SLAM~\cite{zhang2023go}
& Spann3r~\cite{wang20243d} 
& Slam3r (Ours) \\

\toprule

FPS $\uparrow$ 
& $\sim$20
& $\sim$8
& {\textgreater50} 
& $\sim$20 \\

\bottomrule
\end{tabular}

}
\caption{
Comparison of running time efficiency. This table reports only competitors achieving more than 5 FPS. 
}
\label{tab:fps}
\end{table}


